C-SHORe: Higher-Order Verification via Collapsible Pushdown System Saturation

Higher-order recursion schemes (HORS) have received much attention as a useful abstraction of higher-order functional programs with a number of new verification techniques employing HORS model-checking as their centrepiece. We give an account of the C-SHORe tool, which contributed to the ongoing quest for a truly scalable model-checker for HORS by offering a different, automata theoretic perspective. C-SHORe implements the first practical model-checking algorithm that acts on a generalisation of pushdown automata equi-expressive with HORS called collapsible pushdown systems (CPDS). At its core is a backwards saturation algorithm for CPDS. Additionally, it is able to use information gathered from an approximate forward reachability analysis to guide its backward search. Moreover, it uses an algorithm that prunes the CPDS prior to model-checking and a method for extracting counter-examples in negative instances. We provide an up-to-date comparison of C-SHORe with the state-of-the-art verification tools for HORS. The tool and additional material are available from http://cshore.cs.rhul.ac.uk.

==> stack-automata-properties.tex <==
% Stack automata properties appearing in LMCS paper

\subsubsection{Properties of Stack Automata}

We show here that stack automata membership is linear time, while emptiness is
PSPACE.  These are standard complexities for alternating finite word automata.

Several further results can also be shown~\cite{BCHS12}, which we have omitted for space reasons: the sets of stacks accepted
by these automata form an effective Boolean algebra (note that complementation
causes a blow-up in the size of the automaton); and they accept the same family
of collapsible stacks as the automata used by Broadbent\etal~\cite{BCOS10}.  We
omit these here for space reasons.



\begin{prop}[Stack Automata Membership]
    Membership of order-$\cpdsord$ stack automata can be tested in linear time
    in the size of the input stack and stack automaton.
\end{prop}
\proof
    Take a stack $\stackw$ and let
    \[
    \saauta = \tuple{
                  \sastates_\cpdsord,\ldots,\sastates_1,
                  \alphabet,
                  \sadelta_\cpdsord,\ldots,\sadelta_1,
                  \safinals_\cpdsord, \ldots,\safinals_1
              } \ .
    \]

    The membership algorithm iterates from the bottom (end) of the stack to the top (beginning).
    Take the graph representing $\stackw$.
    We start by labelling the final node with the set $\safinals_\cpdsord$.  It
    is easy to verify at all stages that if the label of a node contains a state
    $\sastate$, then the stack from that node is in $\slang{\sastate}{\saauta}$.
    Now, suppose we have labelled up to a given node.  For convenience, we will
    refer to nodes by their labelled state set, and we show, by cases, how to
    label the preceding node with a state-set $\sastateset_0$.

    In the first case, we have node $\sastateset_1$ connected to $\sastateset_0$
    by a $\sclose{\opord}$ character.  That is
    \begin{center}
%BEGIN IMAGE
        \begin{psmatrix}[nodealign=true,colsep=2ex,rowsep=2ex]
            \rnode{N0}{$\sastateset_0$} && \rnode{N1}{$\sastateset_1$} &&
            $\cdots$

            \psset{nodesep=.5ex}
            \ncline{->}{N0}{N1}^{$\sclose{\opord}$}
        \end{psmatrix}
%END IMAGE
%HEVEA\imageflush
    \end{center}
    where $\sastateset_0$ is the set $\safinals_\opord$.  This is because
    $\sastateset_0$ labels the end of an order-$\opord$ stack.

    In the next case the connection is by a character $\cha$ with a collapse link
    and we have
    \begin{center}
        \vspace{2ex}
%BEGIN IMAGE
        \begin{psmatrix}[nodealign=true,colsep=2ex,rowsep=2ex]
            \rnode{N0}{$\sastateset_0$} &\pnode{N01}&
            \rnode{N1}{$\sastateset_1$} && $\cdots$ &&
            \rnode{N2}{$\sastateset_\branch$} && $\cdots$ \ .\\

            \psset{nodesep=.5ex,angle=-90,linearc=.2}
            \ncline{->}{N0}{N1}^{$\cha$}
            \ncbar[nodesepA=0]{->}{N01}{N2}
        \end{psmatrix}
%END IMAGE
%HEVEA\imageflush
    \end{center}
    where $\sastateset_0 = \setcomp{\sastate}{\sastate
    \satrancol{\cha}{\sastateset'_\branch} \sastateset'_1 \in \sadelta_1 \land
    \sastateset'_1 \subseteq \sastateset_1 \land \sastateset'_\branch \subseteq
    \sastateset_\branch}$.  Thus, any state in $\sastateset_0$ has a transition to
    states from which the remainder of the stack is accepted.

    In the final case we have
    \begin{center}
        \vspace{2ex}
%BEGIN IMAGE
        \begin{psmatrix}[nodealign=true,colsep=2ex,rowsep=2ex]
            \rnode{N0}{$\sastateset_0$} && \rnode{N1}{$\sastateset_1$} &&
            \rnode{N2}{$\cdots$} && \rnode{N3}{$\sastateset_2$} && $\cdots$

            \psset{nodesep=.5ex}
            \ncline{->}{N0}{N1}^{$\sopen{\opord}$}
            \ncline{->}{N2}{N3}^{$\sclose{\opord}$}
        \end{psmatrix}
%END IMAGE
%HEVEA\imageflush
    \end{center}
    where $\sclose{\opord}$ matches $\sopen{\opord}$.  We define $\sastateset_0
    = \setcomp{\sastate}{\sastate \satran{\sastate'} \sastateset \in
    \sadelta_{\opord+1} \land \sastate' \in \sastateset_1 \land \sastateset
    \subseteq \sastateset_2}$.  Thus, there is a state $\sastate \in
    \sastateset_0$ whenever there is a transition $\sastate \satran{\sastate'}
    \sastateset$ such that the next order-$\opord$ stack is accepted from
    $\sastate'$ and the remainder of the stack is accepted from $\sastateset$.

    Thus, after this labelling, we can test whether $\stackw \in
    \slang{\sastateset_0}{\saauta}$ for $\sastateset_0 \subseteq
    \sastates_\opord$ by checking whether $\sastateset_0 \subseteq \sastateset$
    where $\sastateset$ labels the node containing the first $\sopen{\opord-1}$
    character of the word, or if $\opord = 1$, the first character $\cha \in
    \alphabet$.
\qed

We now show that emptiness checking is PSPACE-complete.

\begin{prop}[Emptiness of Stack Automata]
    Given an order-$\cpdsord$ stack automaton $\saauta$ and a state $\sastate$
    of $\saauta$, deciding if there is some $\stackw \in
    \slang{\sastate}{\saauta}$ is PSPACE-complete.
\end{prop}
\proof
The problem is already PSPACE-hard for alternating word automata which correspond to the order-1 case \cite{Chandra81}. We now establish the upperbound.

    Let $\saauta = \tuple{
                  \sastates_\cpdsord,\ldots,\sastates_1,
                  \alphabet,
                  \sadelta_\cpdsord,\ldots,\sadelta_1,
                  \safinals_\cpdsord, \ldots,\safinals_1
              }
$ be a stack automaton. We use a fixed point to compute
the set $\sastates_{ac} = \{ \, q \in \sastates_{k} \mid \slang{q}{\saauta} \neq \emptyset \,\}$.

For this, we take $Q_{0}$ to be the set of all final states. For all
$i \geq 0$, we define $Q_{i+1}$ by adding to $Q_{i}$ all states $q \in \sastates_{k}$
such that:
\begin{itemize}
\item for $k>1$, there exists a transition $q
\satrancol{q'}{} {Q} \in \sadelta_{k}$ with $Q \subseteq  Q_{i}$ and $q' \in Q_{i}$.
\item for $k=1$, there exists a transition $\sastate
    \satrancol{\cha}{\sastateset_\branch} \sastateset \in \sadelta_1$ with
$Q,Q_{\branch} \subseteq Q_{i}$.
\end{itemize}

As the sequence of the $Q_{i}$ is increasing (for inclusion), we have
$Q_{j+1}=Q_{j}$ for some index $j \geq 0$. We claim that $Q_{j}$ is the set
$Q_{ac}$. A straightforward induction shows that for all $i$ we have $Q_{i} \subseteq Q_{ac}$ and
hence $Q_{j} \subseteq Q_{ac}$.

Assume toward a contradiction, that the converse
inclusion does not hold. Let $\stackw$ be smallest stack accepted by a state $q \in
\sastates_{k} \setminus Q_{j}$. If $k = 1$, then $\stackw = \ccompose{\cha^{\tuple{\opord,\idxi'}}}{1}{\stackw'}$
and there exists a transition $\sastate \satrancol{\cha}{\sastateset_\branch}
\sastateset \in \sadelta_1$ with $w'$ accepted from $Q$ and $u$ is accepted from
$Q_{\branch}$ where $u=\apply{\collapse{\opord}}{\stackw}$. As $q$ does not belongs to $Q_{j}$, then either $u$ or $w'$ is
accepted from a state not in $Q_{j}$. As $u$ and $w'$ are both smaller than $w$,
this contradicts the definition of $w$. The case $k>1$ is similar.

The algorithm to test emptiness from a given state $p \in \sastates_\cpdsord$
consists of computing $Q_{j}$ by iteratively computing the $Q_{i}$ and then
checking if $p$ belongs to $Q_{j}$.
\qed



